Efficient Record-and-Replay Arithmetic for Quantum Elliptic-Curve Point Addition

We study reversible secp256k1 point-addition circuits developed through ECDSA.Fail for Shor's elliptic-curve discrete-logarithm algorithm. Two complementary constructions improve record-and-replay GCD arithmetic: Jump-2 groups binary-GCD steps and compresses their decisions using base-5 encoding, while ping-pong uses fixed register alternation and one-bit decisions to avoid full-width comparisons and data-dependent swaps. Fused replay combines doubling and signed addition into one modular correction. Both constructions support quantum-addressed window selection with measurement-based lookup cleanup. We compare three circuits on 100,000 fresh inputs across nine lookup-table configurations. A separately tested repair uses 1,419 qubits and 1.356 million mean executed Toffolis, with no detected failures on another 100,000 inputs. Structured supported-input counterexamples remain, so these tests do not establish all-input correctness. We also provide conditional coherent-error analysis and reversible safegcd comparisons. Under the stated window allowance, repaired-circuit resources lie below Google's low-gate caps and Schrottenloher's low-gate estimates, but differing accounting and correctness evidence preclude formal dominance. The results concern individual window-selected additions, not complete Shor computations.

==> evidence/fresh-strata-table.tex <==
\begin{table}[tbp]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Table stratum & Inputs & Original PP & Conservative PP & Jump-2 \\
\midrule
$B=G,\ i=0$ & $11{,}111$ & $8$ & $0$ & $18$ \\
$B=G,\ i=128$ & $11{,}111$ & $2$ & $0$ & $20$ \\
$B=G,\ i=240$ & $11{,}111$ & $6$ & $0$ & $27$ \\
$B=P_1,\ i=0$ & $11{,}111$ & $6$ & $0$ & $26$ \\
$B=P_1,\ i=128$ & $11{,}111$ & $5$ & $0$ & $19$ \\
$B=P_1,\ i=240$ & $11{,}111$ & $2$ & $0$ & $19$ \\
$B=P_2,\ i=0$ & $11{,}111$ & $6$ & $0$ & $30$ \\
$B=P_2,\ i=128$ & $11{,}111$ & $1$ & $0$ & $31$ \\
$B=P_2,\ i=240$ & $11{,}112$ & $3$ & $0$ & $25$ \\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{Any-channel failures by fresh table stratum, with $\mathcal T_B^{(i)}[j]=[j2^i]B$. Each row uses the same inputs for all three circuits. Stratum-specific Wilson intervals and paired discordances are included in the analysis JSON.}
\label{tab:fresh-strata}
\end{table}


==> evidence/fresh-validation-summary.tex <==
No output, phase, or ancilla failures were detected for the conservative variant on the $100{,}000$ fresh cases. Original ping-pong and Jump-2 have $39$ and $215$ any-channel failures. All three circuits pass the $3$ retained identity-addend cases. No additional generic-domain exception occurs.

Relative to original ping-pong, the conservative configuration adds $54$ qubits, $11.12\%$ mean Toffoli work, and $15.60\%$ raw $QT$. Relative to Jump-2, it uses $230$ more qubits and $17.74\%$ fewer mean Toffolis, with $1.46\%$ lower raw $QT$. These are complete-circuit comparisons at different observed error rates, not equal-error optima. Counted Clifford work is $10.34\%$ higher than Jump-2.

The per-call sensitivity proxies $QT/\hat p$ are $\freshBaseRetry$B, $\freshConservativeRetry$B, and $\freshJumpRetry$B for original ping-pong, conservative ping-pong, and Jump-2. They do not estimate retries inside a coherent computation.


==> evidence/shared-accuracy-table.tex <==
\begin{table}[tbp]
\centering\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}lrrrrl@{}}
\toprule
Circuit & cls & pha & anc & any & $95\%$ error interval \\
\midrule
Jump-2 mixed & 154 & 115 & 0 & 192 & $[0.1667\%,0.2211\%]$ \\
Source parent mixed & 216 & 169 & 0 & 267 & $[0.2369\%,0.3010\%]$ \\
Ping-pong mixed & 35 & 17 & 0 & 42 & $[0.0311\%,0.0568\%]$ \\
Jump-2 replay & 151 & 117 & 0 & 191 & $[0.1658\%,0.2200\%]$ \\
Ping-pong replay & 33 & 14 & 0 & 36 & $[0.0260\%,0.0498\%]$ \\
Jump-2 split & 151 & 122 & 0 & 192 & $[0.1667\%,0.2211\%]$ \\
Ping-pong split & 33 & 15 & 0 & 35 & $[0.0252\%,0.0487\%]$ \\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{Full-channel outcomes on the same $100{,}000$ inputs. Categories overlap. The two unsupported identity rows fail in each mixed circuit and pass in each windowed circuit. Wilson intervals describe sampling uncertainty, not coherent error.}
\label{tab:shared-accuracy}
\end{table}


==> evidence/shared-resources-table.tex <==
\begin{table}[tbp]
\centering\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Circuit & $Q$ & Mean $T$ (M) & $QT$ (B) & $QT/\hat p$ (B) \\
\midrule
Jump-2 mixed & $1{,}151$ & $1.299441$ & $1.495656$ & $1.498534$ \\
Source parent mixed & $1{,}150$ & $1.284771$ & $1.477486$ & $1.481442$ \\
Ping-pong mixed & $1{,}321$ & $0.952719$ & $1.258542$ & $1.259071$ \\
Jump-2 replay & $1{,}162$ & $1.684161$ & $1.956995$ & $1.960740$ \\
Ping-pong replay & $1{,}338$ & $1.288560$ & $1.724093$ & $1.724714$ \\
Jump-2 split & $1{,}162$ & $1.523120$ & $1.769866$ & $1.773271$ \\
Ping-pong split & $1{,}338$ & $1.127527$ & $1.508631$ & $1.509160$ \\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{Resources on the shared $100{,}000$-input corpus. M and B denote $10^6$ and $10^9$. Means include failures and the two identity rows. Mixed circuits do not support those identity rows. Replay and split denote the window-payload cleanup method. The last column is only a per-call sensitivity proxy.}
\label{tab:common-operating-points}
\end{table}


==> figs/fused-replay.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}[x=1cm,y=1cm,
  cell/.style={draw,fill=blue!5,text width=2.25cm,minimum height=1.2cm,align=center,inner sep=3pt,font=\small},
  wire/.style={semithick},flow/.style={->,semithick},
  dot/.style={circle,fill,inner sep=1.3pt}]
  \node[anchor=west,font=\small\bfseries] at (0,6.1) {(a) Ordinary value round and transcript};
  \draw[wire] (0.9,5.55) -- (11.7,5.55);
  \draw[wire] (0.9,4.9) -- (11.7,4.9);
  \draw[wire] (0.9,4.15) -- (11.7,4.15);
  \node[anchor=east,font=\small] at (0.8,5.55) {$s$};
  \node[anchor=east,font=\small] at (0.8,4.9) {$t$};
  \node[anchor=east,font=\small] at (0.8,4.15) {$\ket{0}$};
  \node[dot] at (2,5.55) {};
  \draw[wire] (2,5.55) -- (2,4.15);
  \node[draw,circle,fill=white,inner sep=0pt,minimum size=0.18cm] at (2,4.15) {$\scriptscriptstyle+$};
  \node[dot] at (2.65,4.9) {};
  \draw[wire] (2.65,4.9) -- (2.65,4.15);
  \node[draw,circle,fill=white,inner sep=0pt,minimum size=0.18cm] at (2.65,4.15) {$\scriptscriptstyle+$};
  \node[font=\scriptsize,anchor=south] at (2,5.62) {$s[1]$};
  \node[font=\scriptsize,anchor=south] at (2.65,4.98) {$t[1]$};
  \node[cell,text width=3.4cm,minimum height=1.1cm] (update) at (6.2,5.225) {$s\gets s$\\$t'=(t+(-1)^e s)/2$};
  \node[dot] at (6.2,4.15) {};
  \draw[wire] (6.2,4.15) -- (update.south);
  \node[fill=white,font=\small,inner sep=2pt] at (9.7,4.15) {$e=t[1]\oplus s[1]$};
  \node[fill=white,font=\small,inner sep=2pt] at (10.2,4.9) {$t'$};
  \node[font=\scriptsize,anchor=west] at (0.9,3.72) {The target alternates. Reverse value computation later clears the recorded bit.};
  \node[anchor=west,font=\small\bfseries] at (0,3.38) {(b) Inverse payload replay: $z\gets2z+(-1)^\sigma y\pmod p$, $\sigma=1-e$};
  \node[anchor=west,font=\small] at (0,2.95) {Fused};
  \node[anchor=east,font=\small] at (11.7,2.95) {$308+57+28=393$};
  \node[cell] (fd) at (1.35,2.05) {Double, retain $d$\\Clifford only};
  \node[cell] (fa) at (4.3,2.05) {Signed word add\\$256+52$};
  \node[cell,fill=orange!10] (ff) at (7.25,2.05) {One fold $\kappa F$\\$54+3$};
  \node[cell] (fe) at (10.2,2.05) {Clear $d$ by parity\\Clear $o$: $28$};
  \draw[flow] (fd.east) -- (fa.west);
  \draw[flow] (fa.east) -- node[above,font=\scriptsize] {$d,o$} (ff.west);
  \draw[flow] (ff.east) -- (fe.west);
  \node[anchor=west,font=\small] at (0,1.03) {Unfused, matched fold width};
  \node[anchor=east,font=\small] at (11.7,1.03) {$55+308+55+28=446$};
  \node[cell,fill=orange!10] (ud) at (1.35,0.05) {Double and fold\\$55$};
  \node[cell] (ua) at (4.3,0.05) {Signed word add\\$256+52$};
  \node[cell,fill=orange!10] (uf) at (7.25,0.05) {Fold add carry\\$55$};
  \node[cell] (ue) at (10.2,0.05) {Clear add carry\\$28$};
  \draw[flow] (ud.east) -- (ua.west);
  \draw[flow] (ua.east) -- (uf.west);
  \draw[flow] (uf.east) -- (ue.west);
\end{tikzpicture}
\caption{Value control and source-counted inverse payload replay. Panel (a) records the low-bit XOR with two CNOTs. Panel (b) excludes the value round, initialization, and transcript cleanup. Its word addition includes $52$ Toffolis for chunk-boundary phase comparisons, and carry erasure retains its $28$-Toffoli phase comparison. Matching the $56$-bit fold does not establish identical failure sets.}
\label{fig:fused-inverse-replay}
\end{figure}


==> figs/resource-frontier.tex <==
\begin{figure}[H]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
  \begin{axis}[name=hist,width=6.0cm,height=5.4cm,xmode=log,ymode=log,
    xmin=800,xmax=1450,ymin=800000,ymax=700000000,
    xlabel={Peak logical qubits $Q$},ylabel={Executed Toffoli count $T$},
    title={Historical mixed circuits},
    xtick={825,1151,1321},xticklabels={825,1151,1321},
    ytick={1000000,10000000,100000000,500000000},
    yticklabels={1M,10M,100M,500M},log ticks with fixed point,
    axis lines=left,grid=major,grid style={black!10},
    tick label style={font=\footnotesize},label style={font=\small},
    title style={font=\small},
    legend style={at={(0.5,-0.32)},anchor=north,draw=none,font=\scriptsize},
    legend cell align=left]
    \addplot[black,thick,mark=*,mark size=1.8pt]
      table[x=qubits,y=toffoli,col sep=comma]{evidence/cutoff-pareto.csv};
    \addlegendentry{July cutoff}
    \addplot[only marks,mark=square*,mark size=2.7pt,color=orange!80!black]
      coordinates {(\resPMixedPlotQ,\resPMixedPlotT)};
    \addlegendentry{Later ping-pong, shared corpus}
  \end{axis}
  \begin{axis}[at={(hist.east)},anchor=west,xshift=1.25cm,width=6.0cm,height=5.4cm,
    xmin=1100,xmax=1400,ymin=900000,ymax=1850000,
    xlabel={Peak logical qubits $Q$},ylabel={$T$ on shared corpus},
    title={Windowed cleanup comparison},
    xtick={1162,1250,1338},xticklabels={1162,1250,1338},
    ytick={1000000,1200000,1400000,1600000,1800000},
    yticklabels={1.0M,1.2M,1.4M,1.6M,1.8M},scaled y ticks=false,
    axis lines=left,grid=major,grid style={black!10},
    tick label style={font=\footnotesize},label style={font=\small},
    title style={font=\small}]
    \addplot[only marks,mark=o,mark size=3pt,color=blue!65!black]
      coordinates {(\resJReplayPlotQ,\resJReplayPlotT)};
    \addplot[only marks,mark=*,mark size=3pt,color=blue!65!black]
      coordinates {(\resJSplitPlotQ,\resJSplitPlotT)};
    \draw[->,thick,blue!65!black] (axis cs:1162,1668000) -- (axis cs:1162,1540000);
    \node[font=\scriptsize,anchor=south] at (axis cs:1162,1710000) {Jump-2};
    \node[font=\scriptsize,anchor=west] at (axis cs:1175,1597000) {$-9.56\%$};
    \addplot[only marks,mark=diamond,mark size=3.5pt,color=teal!75!black]
      coordinates {(\resPReplayPlotQ,\resPReplayPlotT)};
    \addplot[only marks,mark=diamond*,mark size=3.5pt,color=teal!75!black]
      coordinates {(\resPSplitPlotQ,\resPSplitPlotT)};
    \draw[->,thick,teal!75!black] (axis cs:1338,1271000) -- (axis cs:1338,1144000);
    \node[font=\scriptsize,anchor=south] at (axis cs:1338,1320000) {Ping-pong};
    \node[font=\scriptsize,anchor=east] at (axis cs:1325,1207000) {$-12.50\%$};
  \end{axis}
\end{tikzpicture}%
}
\caption{Left: the historical July mixed-addition frontier across the challenge's resource tracks, together with the later mixed ping-pong measurement. Right: matched-corpus windowed cleanup comparisons, from hollow replay markers to filled split markers at fixed $Q$. The panels separate interfaces and validation settings rather than claiming a universal equal-error frontier.}
%\caption{Left: the historical July mixed-addition frontier and later mixed ping-pong measurement. Right: matched-corpus windowed cleanup comparisons, from hollow replay markers to filled split markers at fixed $Q$. The panels separate interfaces and evidence rather than claiming a universal equal-error frontier.}
\label{fig:frontier-reconstruction}
\end{figure}


==> sections/08-acknowledgments.tex <==
\section*{Acknowledgments}

We thank Craig Gidney and Tanuj Khattar of Google Quantum AI for carefully reviewing earlier drafts of this manuscript and for their constructive comments and suggestions, which substantially improved its technical accuracy, clarity, and presentation. We also thank Joe Doyle of Trail of Bits for his helpful suggestions and insightful discussions. Any remaining errors are our own.

==> sections/09-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

The ping-pong construction trades a longer transcript for simpler reversible control and cheaper modular replay. Its isolated cell comparison gives an $11.9\%$ static-Toffoli saving at matched fold width. A controlled backend experiment retains a $340{,}442$-Toffoli saving with the Karatsuba square fixed and post-emission passes disabled. Live-allocation and phase ledgers identify the corresponding memory and arithmetic costs. These cost results do not equalize the configurations' correctness guarantees, and the termination argument concerns the ideal recurrence rather than the finite-width implementation.

Both ping-pong and Jump-2 support single-call window-selected addition with exact lookup cleanup. The fresh validation study evaluates their resource--error trade-offs after freezing the circuits and analysis. The conservative ping-pong variant uses $Q=\freshConservativeQ$ and $T\approx\freshConservativeTM$ million, with $\freshConservativeAny$ detected failures on $100{,}000$ inputs. Original ping-pong uses fewer resources but has $\freshBaseAny$ failures on the same inputs. Jump-2 uses fewer qubits than conservative ping-pong but has a higher mean Toffoli count and $\freshJumpAny$ detected failures.

These results connect source-level arithmetic savings to reproducible single-call evidence. Their development combined human research, agent-assisted implementation, and public validation. Establishing a composed Shor error budget still requires stronger arithmetic guarantees and validation of the complete schedule. The reported costs are not complete fault-tolerant attack estimates.


==> unused/low-width-circuits.tex <==
\section{Low-Width Point-Addition Circuits}
\label{sec:best-low-Q-circuit}

The historical circuit \texttt{b6f2b0a} provides a complementary low-width operating point. It replaces the dialog transcript with register-shared extended Euclidean inversion and reaches $825$ qubits at approximately $489$ million Toffolis. Unlike the main windowed results, it has not received the new shared-corpus evaluation or coherent table adaptation.

\subsection{Register-Shared Euclidean Inversion}
\label{sec:register-shared-eea}

The storage-sharing principle originates with Proos and Zalka~\cite{proos-zalka03}. Luo et al.~\cite{luo26} supplied the explicit two-register construction used here. Shrinking remainders and growing cross-cofactors share storage, with quotient fields and alignment metadata.

For denominator $x\neq0$, let $\rho,\rho'$ be remainders, $c,c'$ cross-cofactors, and $\pi$ their orientation bit. Initially $(\rho,\rho',c,c',\pi)=(p,x,1,0,0)$, with invariants
\begin{equation}
  \begin{aligned}
    \rho c+\rho'c'&=p,\\
    \rho&\equiv(-1)^{\pi+1}xc'\pmod p,\\
    \rho'&\equiv(-1)^\pi xc\pmod p.
  \end{aligned}
  \label{eq:register-shared-cross-invariants}
\end{equation}
For $\kappa=2^{\ell_s}$, the subtractive microstep is
\begin{equation}
  \rho\gets\rho-\kappa\rho',
  \qquad c'\gets c'+\kappa c.
  \label{eq:register-shared-microstep}
\end{equation}
The opposite signs preserve all three invariants. Exchanging primed and unprimed roles updates $\pi$.

Two physical banks pack the active fields:
\begin{equation}
  W_1=c\Vert q\Vert\rho,
  \qquad W_2=\operatorname{rot}_{\ell_s}(c'\Vert\rho').
  \label{eq:register-shared-layout}
\end{equation}
Here $q$ is the partial quotient and $\Vert$ denotes concatenation. Rotation aligns fields without a shifted copy. Quotient bits occupy released remainder space. Each bank has $n+3=259$ qubits.

The circuit executes $1{,}479$ microsteps, including termination padding. At the normalized endpoint $\rho=1$, $\rho'=q=0$, the invariant gives $c'\equiv(-1)^{\pi+1}x^{-1}\pmod p$. Sign correction and multiplication produce the quotient. Reversal restores the denominator and clears the inversion state.

\subsection{Lifetime Refinements and Alternate-Witness Cleanup}
\label{sec:low-qubit-lifetimes}

The source uses $\widetilde d_x=x_A-x_R=-d_x$ and $\widetilde d_y=y_A-y_R=-d_y$, preserving the slope ratio. Division retains $\lambda=\widetilde d_y\widetilde d_x^{-1}$ separately while restoring both differences, instead of overwriting the numerator as in \Cref{fig:best-qxt-circuit-pipeline}.

Next, $Y\gets Y-\lambda X=0$ releases the numerator register for squaring and coordinate updates. After producing $x_{R'}=\lambda^2-x_R-x_A$, the circuit constructs
\begin{equation}
  d_x'=x_A-x_{R'},
  \qquad d_y'=\lambda d_x'=y_{R'}+y_A.
  \label{eq:low-q-output-witness}
\end{equation}
A second register-shared division erases the retained slope using $d_y'(d_x')^{-1}=\lambda$. Finally, $X\gets x_A-d_x'$ and $Y\gets d_y'-y_A$ recover $R'$. Both divisions require the generic-affine domain of \Cref{sec:task}.

The two EEA stages determine the peak:
\begin{equation}
  \underbrace{259+259}_{\text{EEA banks}}+
  \underbrace{257}_{\text{coordinate}}+
  \underbrace{37}_{\text{metadata}}+
  \underbrace{13}_{\text{workspace}}=825.
  \label{eq:low-q-peak}
\end{equation}
Inactive fields temporarily hold comparison, carry, and rotation controls. The final $826$-to-$825$ reduction reconstructs one omitted quotient-length bit locally.

These are simultaneous physical allocations, not separate worst-case widths. The invariants and alternate-witness identity are exact, but the submitted active widths and guards remain empirically calibrated. The $825$-qubit count therefore has a different validation scope from the windowed results that follow.

